Efficient Methods and Parallel Execution for Algorithm Sensitivity Analysis with Parameter Tuning on Microscopy Imaging Datasets

Background: We describe an informatics framework for researchers and clinical investigators to efficiently perform parameter sensitivity analysis and auto-tuning for algorithms that segment and classify image features in a large dataset of high-resolution images. The computational cost of the sensitivity analysis process can be very high, because the process requires processing the input dataset several times to systematically evaluate how output varies when input parameters are varied. Thus, high performance computing techniques are required to quickly execute the sensitivity analysis process. Results: We carried out an empirical evaluation of the proposed method on high performance computing clusters with multi-core CPUs and co-processors (GPUs and Intel Xeon Phis). Our results show that (1) the framework achieves excellent scalability and efficiency on a high performance computing cluster -- execution efficiency remained above 85% in all experiments; (2) the parameter auto-tuning methods are able to converge by visiting only a small fraction (0.0009%) of the search space with limited impact to the algorithm output (0.56% on average). Conclusions: The sensitivity analysis framework provides a range of strategies for the efficient exploration of the parameter space, as well as multiple indexes to evaluate the effect of parameter modification to outputs or even correlation between parameters. Our work demonstrates the feasibility of performing sensitivity analyses, parameter studies, and auto-tuning with large datasets with the use of high-performance systems and techniques. The proposed technologies will enable the quantification of error estimations and output variations in these pipelines, which may be used in application specific ways to assess uncertainty of conclusions extracted from data generated by these image analysis pipelines.

==> motivating.tex <==
\subsection{Motivating Application Domain} \label{sec:app}
%
High-resolution microscopy imaging of tissue specimens enables the study of disease at the cellular
and sub-cellular levels. Characterizing the sub-cellular morphology of tissue can 
lead to a better understanding of disease mechanisms and a better assessment 
of response to treatment. It is increasingly becoming feasible, with wider availability 
of advanced tissue scanners at lower price points, for research studies to collect 
tens of thousands of high resolution images. A contemporary digital microscopy scanner can 
capture a whole slide tissue image containing 20 billion pixels (using 40X objective 
magnification) in a few minutes.  A scanner with a slide loader and auto-focusing mechanism 
can generate hundreds of images in one or two days. 

\begin{table*}[htb!]
\begin{center}
\vspace*{-2ex}
\caption{Parameters their value ranges for two example workflows.}
%\vspace*{-2ex}
\begin{scriptsize}
\subtable[Parameters of the Watershed based segmentation workflow. The search space of the segmentation contains about 21 trillion points.]{
\begin{tabular}{l l l l }
\hline
Parameter		& Description   						& Range Value					\\ \hline
Target Image 		& Image used as a normalization target 				& TI $\in [Img1, Img2,...,Img4]$ 		\\ 
Blue(B)/Green(G)/Red(R) & Background detection thresholds 				&  B, G, R $\in [210, 220,...,240]$ 		\\ 
T1/T2			&  Red blood cell detection thresholds				& T1,T2 $\in [2.5,3.0,...,7.5]$			\\ 
G1/G2			&  Thresholds to identify initial the nuclei candidate set	& G1 $\in [5,10,...,80]$ G2 $\in [2,4,...,40]$	\\ 
MinSize			& Filter out objects with area (pixels) smaller than MinSize 		& MinSize $\in [2,4,...,40]$ 			\\ 
MaxSize			& Filter out objects with area larger than MaxSize	 	& MaxSize $\in [900,950,...,1500]$ 		\\ 
MinSizePl		& 	                                                      & MinSizePl $\in [5,10,...,80]$			\\
MinSizeSeg		& Filter out objects with area smaller  than MinSizeSeg 		& MinSizeSeg $\in [2,4,...,40]$ 		\\ 
MaxSizeSeg		& Filter out objects with area smaller than MaxSizeSeg		& MaxSizeSeg $\in [900,950,...,1500]$		\\ 
FillHoles Structure	& Structuring element defining propagation neighborhood		& FillHoles $\in [4$-conn$,8$-conn$]$		\\ 
MorphRecon Structure	& Structuring element defining  propagation neighborhood	& MorphRecon $\in [4$-conn$,8$-conn$]$		\\ 
Watershed Structure	& Structuring element defining  propagation neighborhood	& Watershed $\in [4$-conn$,8$-conn$]$		\\ \hline
\end{tabular}
}
\subtable[Parameters of the Level Set based segmentation workflow. Dummy parameter is used here to account for application output variability
due to its stochastic behaviors. The search space of the segmentation, excluding the dummy parameter contains to 2.8 billion points.]{
\begin{tabular}{l l l l }
\hline
Parameter	& Description   					& Range Value				\\ \hline
Target Image 	& Image used as a normalization target 			& TI $\in [Img1, Img2,...,Img4]$ 	\\ 
OTSU 		& Weighting value applied to the OTSU threshold value	& OTSU $\in [0.1,0.2,...,2.5]$ 		\\ 
Curvature Weight& Curvature weight (CW) of the level set functions	& CW $\in [0.0,0.05,...,1.0]$		\\ 
MinSize		& Minimum object size in micron	per dimension 		& MinSize $\in [1,2,...,20]$ 		\\ 
MaxSize		& Maximum object size in micron	per dimension		& MaxSize $\in [50,55,...,400]$ 	\\ 
MsKernel	& Spatial radius used in the Mean-Shift calculation	& MsKernel $\in [5,6,...,30]$		\\ 
LevetSetIt	& Number of iterations of the level set computation	& LevetSetIt $\in [5,6,...,150]$	\\ 
\end{tabular}
}
\end{scriptsize}
\label{tab:parameters}
%\vspace*{-7ex}
\end{center}
\end{table*}


\begin{figure*}[htb!]
\begin{center}
	\subfigure[fig:water-app][Watershed based segmentation workflow.]{
	\includegraphics[width=\textwidth]{images/nucleiPipelineCur}}
	\subfigure[fig:level-app][Level Set based segmentation workflow.]{
	\includegraphics[width=\textwidth]{images/nucleiPipelineLevelSet}}

\caption{Two example analysis workflows with their cascade of internal
operations. They have the same high level computation stages: normalization,
segmentation and feature computation. The stages of normalization and
feature computation are shared among between the workflows, but different techniques
are used to implement the segmentation phase. The first
(Figure~(a)) uses morphological operations along with watershed
to delineate and separate clumped cells. The second
(Figure~(b)) employs the level set strategy and a mean shift
based clustering to delineate and separate clumped cells}
%\vspace*{-3ex}
\label{fig:example-app}
\end{center}
\end{figure*}

A typical analysis workflow consists of normalization, segmentation, feature
computation, feature refinement and classification operations.  The first three
analysis stages  are typically the most computationally expensive phases of an
analysis run. Figure~\ref{fig:example-app} presents two analysis workflows used
in this work. These workflows share the same high level structure, but
implement the segmentation stage using different strategies. The first
(Figure~\ref{fig:water-app}) uses morphological operations and watershed in the
segmentation~\cite{kong2013machine,kong2016robust,kong2013high}, whereas the second
(Figure~\ref{fig:level-app}) performs the segmentation based on level set and
mean shift clustering. The cascade of operations employed by each of the
workflows are presented in the figures.

Most image analysis workflows are sensitive to variations in input parameters.
A workflow optimized for a group of images or a type of tissue may not perform
well for other tissue types or images. For instance, accurate segmentation of
cancer nuclei is an important image analysis task in digital pathology.
Boundaries of segmented nuclei are algorithm dependent.  Input parameters, such
as the choice of methods for seed selection, intensity thresholds for boundary
detection and thresholds for separation of clumped nuclei, will impact the
results (the number and locations of detected nuclei, the shape of boundaries
of a nucleus, etc). Figure~\ref{fig:two-runs} shows nuclear segmentation
results from two analysis runs. The two analysis pipelines have good agreement
in some regions (i.e., the boundaries of the polygons overlap closely) and
large disagreement in other regions, where either one algorithm has not
segmented nuclei while the other has or there are large differences between the
boundaries of a nucleus segmented by the two algorithms. 


%
\begin{figure*}[htb!]
\begin{center}
\includegraphics[width=0.70\textwidth]{images/two-runs}
%\vspace*{-3ex}
\caption{Nuclear segmentation results from two analysis runs.}
%\vspace*{-3ex}
\label{fig:two-runs}
\end{center}
\end{figure*}

It is, therefore, important to quantify the impact of changes 
in input parameters to output generated by different stages and by the overall workflow.
In this work, we focus on the segmentation stage as our example, because this is a 
crucial stage in extracting morphological information from images and consists of 
several complex and parameterized data transformation steps.

It is challenging to carry out parameter sensitivity analysis and auto-tuning,
even for the segmentation stage, because (1) the number of possible parameter
combinations of an analysis workflow is staggeringly high; (2) the execution of
a single parameter combination may be computationally very demanding depending
on the input dataset. Table~\ref{tab:parameters} presents the parameters of
interest in the segmentation stage for our two use case image analysis
workflows.  The space of parameter values for the watershed and level set based
segmentation contain, respectively, over 21~trillion and 2.8~billion points.
This is even more critical in the context of whole slide tissue image analysis,
because the execution of a single analysis run (i.e., the evaluation of a
single point in the parameter space) can take hours or days depending on the
size of the input dataset. To make sensitivity analyses feasible, it is
necessary: (i)~to propose and utilize effective sensitivity analysis and
auto-tuning methods; and (ii)~to leverage high performance computing techniques
to accelerate these analyses. In the next section we present our proposed
approach to the problem.

%When the target of the analysis is a very large dataset, consisting of tens of
%thousands of images, a single analysis run is usually not sufficient.  The
%effectiveness of an analysis workflow is often sensitive to input data and
%input parameters. This can lead to concerns about with the validity and
%robustness of extracted or discovered morphological properties. It is not
%feasible to manually inspect each dataset for every feature and fine-tune
%analysis workflows in a large-scale analysis effort.  Instead of chiseling out
%a single, optimal ``analysis solution'' through such a labor-intensive process,
%an alternative, more viable approach is to produce ensembles of ``analysis
%solutions'' and compare and evaluate them. This sensitivity analysis process
%can be augmented by parameter tuning. The parameter tuning phase  is often
%carried out by empirically modifying parameters until results approximate a
%reference set of results. The reference set may be, for instance, segmentation
%masks created by a pathologist. 
%
%The parameter tuning and sensitivity analysis processes involve comparing
%results from an analysis run to results from other runs or to a target reference
%output. Examples of comparative operations include (1) evaluation of the
%differences in shape of segmented objects computed by the application to those
%identified in a reference dataset and (2) comparison of feature vectors.  As
%such, a sensitivity analysis or parameter tuning execution for our motivating
%application workflow, presented in Figure~\ref{fig:example-app}, would include
%additional steps to properly execute the comparison operations.
%
%The computation cost of testing each parameter combination and the explosion of
%combinations of parameters values can quickly make it prohibitive to perform an
%exhaustive parameter search to improve application output.
%Table~\ref{tab:parameters} presents the parameters of interest, the description
%and value ranges of the parameters, and the stages of analysis workflow which
%are affected by these parameters in the example application. The parameters and
%value ranges in the table were selected by an application expert. 
%The parameters affect both the normalization and segmentation stages of the
%example application. Their combination creates a parameter search space with
%more than 21~trillion points, which is too large to be completely explored. 


==> queries-complete.tex <==
\subsection{Comparative Analysis} \label{sec:comparative-analysis}
%
Pathology image analysis allows specialists to perform quantitative
measurements of micro-anatomic objects such as nuclei and cells in
high-resolution pathology images and large image datasets. These regions of
micro-anatomic objects are computed through image segmentation algorithms,
represented by their boundaries in a mask. Depending on the application
pipeline, after the segmentation stage, image features can be extracted from
these objects and classified. Quantifying the results of such analysis involves
compute-intensive queries such as spatial cross-matching, overlay of objects,
spatial proximity computations between objects, and global spatial pattern
discoveries. 

We introduce a Comparative Analysis module for the Region Templates Framework
in order to support multiple evaluation metrics for algorithm sensitivity
analysis. In this work we present four different metrics that are used to
evaluate segmentation algorithms. These four metrics are: Diff Pixels, Dice
Coefficient, Mask Intersection Area and the Jaccard Coefficient. The first
metric counts the amount of different pixels from two different masks and the
latter three metrics uses the Hadoop-GIS framework \cite{aji2013hadoop} to
efficiently process complex spatial queries, including spatial cross-matching
and overlay.  These queries are used to compare and evaluate image segmentation
algorithm results by measuring relations between the spatial objects (cells,
veins, etc) from two different masks. Also, these metrics are used in our
auto-tuning framework to iteratively improve the quality of the image analysis
algorithms (Section \ref{sec:auto-tuning}) and consolidate multiple analysis
results from different param-sets to generate more confident results. These
queries often involve billions of spatial objects and heavy geometric
computations \cite{aji2012towards}. Moreover, due to the Hadoop-GIS
integration, applications running under the Region Templates Framework are now
able to use other types of spatial queries, including spatial proximity
computations between objects using Nearest Neighbor Queries (KNN).

%
\subsubsection{Hadoop-GIS Integration} 
%
Hadoop-GIS is a framework capable of parallelizing multiple types of spatial
queries on top of Hadoop's MapReduce. It provides an R*-Tree indexing-driven
spatial query engine to process various types of spatial queries, data
partitioning to achieve task parallelization, implicit query parallelization,
and boundary handling to generate correct results. We used the standalone
library of the Hadoop-GIS Framework in our Comparative Analysis module.

The Hadoop-GIS Framework handles data partitioning by partitioning the data
into tiles, and processing them in parallel. These generated tiles are
considered the unit level for query processing. One major concern when
partitioning data is to avoid high density partitioned tiles that may
eventually cause load imbalance. This concern is handled properly by
recursively breaking high density tiles into smaller ones until a certain
number of objects per tile threshold is met. Another problem that may arise
from partitioning data is splitting an object in distinct tiles
(boundary-handling problem). This problem is solved by using a multiple
assignment approach in which objects that originally would be split, are
replicated and assigned to multiple tiles, followed by a post-processing step
that removes these duplicates in order to remedy the query results. All the
spatial processing performed inside the Hadoop-GIS Framework is handled by a
Real-Time Spatial Query Engine (RESQUE). This engine is able to perform diverse
spatial query types, provide spatial operators and geometric measurement
functions and is also able to run efficiently in a distributed computing
environment. 

In order to execute spatial queries, the Comparative Analysis module extracts
the objects (cells, veins, etc) from the masks and convert them into polygons.
After this process, an application running under Region Templates Framework can
use one of the supported queries to perform spatial processing. The implemented
queries can use the Hadoop-GIS Framework to calculate the intersection area
between the two sets or calculate their spatial proximity. After receiving the
results from the spatial processing engine the Comparative Analyses module may
calculate the Dice Coefficient, Jaccard Index or some other metric in order to
complete the query task.

\subsubsection {Spatial Queries Support} 

The framework supports different kinds
of spatial queries, including spatial join (cross-matching and overlay),
spatial selection (containment query), and aggregation. The integration between
Hadoop-GIS and Region Templates allow the applications running under Region
Templates to use the following four queries to perform spatial processing: Dice
Coefficient Metric, Intersection Area Metric, Jaccard Index Metric, and Nearest
Neighbor Query. The first three metrics are used by the auto-tuning algorithms
to evaluate the segmentation results during the tuning process. The last query
allows application developers to perform spatial proximity computations between
sets of objects, a typical use case scenario of this query is finding out the
features of the cells which are closest to a particular vein or some other
object.

In order to find the intersection area between two spatial datasets, the
polygons from both datasets must be joined by the query engine. The SQL
expression equivalent to this query is discussed in Figure \ref{sql-query}.
Bulk spatial index building using Hilbert R-Tree is performed on each dataset
to generate index files to ensure efficient processing and fast response
\cite{beckmann1990r}. The R*-Tree indexes are small enough to fit in the main
memory. Each tree contains MBBs (Minimum Bounding Boxes) in their inner nodes
and polygons in their leaf nodes. The inner nodes (MBBs) are used to perform
spatial filtering in order to speed-up the join process by comparing the MBBs
instead of the actual polygons. Based on the intersection of the MBBs, the
corresponding polygons are used to perform a more refined geometric
computation. When polygon pairs intersects with each other, the framework
performs spatial measurements to calculate the required results by the query.
These results may be the overlapping area of the intersection, the area of the
union of the polygons or some other spatial measurement.

\begin{figure}[htb!]
\begin{center}
        \includegraphics[width=\textwidth]{images/comparative-analysis}
\vspace*{-1ex}
\caption{Metric Computation Workflow.}
\vspace*{-3ex}
\label{fig:comparative-analysis}
\end{center}
\end{figure}

\paragraph {Dice Coefficient Metric}
This metric is based on the Dice Coefficient, also known as The Sørensen-Dice
index. This coefficient is a statistical metric that ranges from 0 to 1 and is
used to measure the similarity of two samples. The closer to 1 the value of the
metric is, the more similar the samples are. This metric can be calculated by
dividing the intersection area of two samples by the sum of their respective
areas.

\paragraph {Mask Intersection Metric} We developed this metric to represent the
percentual relation between the area of the intersection between two samples
divided by the area of the reference mask set. It is similar to the overlap
coefficient but instead of dividing the intersection area by the smallest set,
we divide it by the reference set. In our use case, the reference set is
usually the largest set of polygons. They correspond to the objects of the
reference mask that were marked by a pathologist.

\paragraph {Jaccard Index Metric} The Jaccard Index also ranges from 0 to 1 and
is very similar to the Dice Coefficient, however they are not equivalent
because the triangle inequality isn't satisfied. The Jaccard Index is
considered to be a semimetric of the Dice Coefficient. The Jaccard Index is
calculated by dividing the intersection area between two sets by the union area
of these sets.

%\begin{lstlisting}[
%           language=SQL,
%           showspaces=false,
%           basicstyle=\scriptsize\upshape\ttfamily,
%           numbers=left,
%           numberstyle=\tiny,
%          label=sql-query,
%          caption=An equivalent SQL query to the Jaccard Index Metric.]
%SELECT
% ST_AREA (ST_INTERSECTION (ta.polygon, tb.polygon))/
% ST_AREA (ST_UNION (ta.polygon, tb.polygon)) 
%  AS JaccardIndex,
%FROM markup_polygon ta JOIN markup_polygon tb ON
% ST_INTERSECTS( ta.polygon, tb.polygon) = TRUE
%WHERE ta.provenance='MASK1' AND tb.provenance='MASK2';
%\end{lstlisting}
\begin{figure}%[htb!]
\begin{center}
        \includegraphics[width=\textwidth]{images/sql-query}
\vspace*{-1ex}
\caption{An equivalent SQL query to the Jaccard Index Metric.}
\vspace*{-3ex}
\label{fig:sql-query}
\end{center}
\end{figure}

\paragraph {Nearest Neighbor Query}

Nearest neighbor (KNN) search in analytical imaging analysis can be
computationally expensive, we use Hadoop-GIS to efficiently perform these
queries in order to understand correlations between spatial proximity and cell
features. The implemented query allows selecting the K nearest objects or
within a certain bound. A typical scenario that a pathologist can use this
query is to find the nearest objects (blood vessels, cells, etc) for each cell
of a given set.

